A Cut Principle for Information Flow

We view a distributed system as a graph of active locations with unidirectional channels between them, through which they pass messages. In this context, the graph structure of a system constrains the propagation of information through it. Suppose a set of channels is a cut set between an information source and a potential sink. We prove that, if there is no disclosure from the source to the cut set, then there can be no disclosure to the sink. We introduce a new formalization of partial disclosure, called *blur operators*, and show that the same cut property is preserved for disclosure to within a blur operator. This cut-blur property also implies a compositional principle, which ensures limited disclosure for a class of systems that differ only beyond the cut.

==> collapse.tex <==
\section{Collapsing frames}
\label{sec:collapse}

A \emph{collapse} function is a homomorphism between two frames.  We
are interested in collapse functions because \emph{frame refinement
  steps} are inverse to them.  That is, we can regard a relation
between two frames as a refinement if its inverse is a homomorphism.
We focus on a form of refinement in which the structure of the frame
is refined, but the set of executions is essentially unchanged.

\begin{definition}
  \label{def:collapse}
  Suppose given frames $\Frame=(\Locations,\Channels,\mathcal
  {D},\pends,\ldots)$ and $\Frame'=(\Locations',\Channels',\mathcal
  {D}',\pends',\ldots)$.  Let $h=(h_L,h_C,h_D)$, where
  % 
  $ h_L\colon\Locations\rightarrow\Locations'$,
  $h_C\colon\Channels\rightarrow\Channels'$, and 
  $h_D\colon\mathcal{D}\rightarrow\mathcal{D}'$.
%
  We apply $h$ to values by using the relevant component.
  \begin{enumerate}
    \item $h$ is a \emph{graph homomorphism}
    $h\colon\Frame\rightarrow\Frame'$ iff, for all $\ell\in\Locations$
    and $c\in\Channels$,
%
    \begin{eqnarray*}
      \entry(c)\in\pends(\ell)&\mathrm{implies} &
      \entry(h(c))\in\pends(h(\ell)) \\
      \exit(c)\in\pends(\ell)& \mathrm{implies} &
      \exit(h(c))\in\pends(h(\ell)) .
    \end{eqnarray*}
%
%       \item $c\in\Channels$ is an $h$\emph{-self-loop} iff
%       $\sender(h(c))=\recipt(h(c))$.
%
    \item Let $h\colon\Frame\rightarrow\Frame'$, $\bnd\in\ES(\Frame)$,
    and $\bnd'\in\ES(\Frame')$.  $\bnd'$ is an $h$\emph{-image} of
    $\bnd$ iff for some $\preceq$-preserving bijection
    $\phi\colon\events(\bnd)\rightarrow\events(\bnd')$, for all
    $e\in\events(\bnd)$, 
%
    $$\chan(\phi(e))=h(\chan(e))\quad\mathrm{and} \quad
    \msg(\phi(e))=h(\msg(e)).$$
%
    Observe that any two $h$-images of $\bnd$ are isomorphic to each
    other.  We will write $h(\bnd)$ for any $h$-image of $\bnd$, if
    any exists.
    \item A graph homomorphism $h\colon\Frame\rightarrow\Frame'$ is a
    \emph{frame homomorphism} iff:
    \begin{enumerate}
      \item for every $\bnd\in\exec(\Frame)$, there exists an $h$-image
      $h(\bnd)\in\exec(\Frame')$; \label{cl:collapse:forward} and 
      \item for every $\bnd'\in\exec(\Frame')$, $\bnd'=h(\bnd)$ for
      \label{cl:collapse:backward}
      some $\bnd\in\exec(\Frame)$.  \defend
    \end{enumerate}
%
  \end{enumerate}
%
\end{definition}
%
\begin{lemma}\label{lemma:frame:hom}
  If $\bndA\in\exec(\Frame)$ and $C\subseteq\Channels$, then
  $h(\restrict{\bndA}C)=\restrict{h(\bndA)}{h(C)}$.  
\end{lemma}
%
With our definitions, security properties are preserved under
collapse; i.e.~insecurity (information flow) is preserved under
refinement.
%
\begin{theorem}
  \label{thm:morphisms:preserve:blur}
  Let $h\colon\Frame\rightarrow\Frame'$ be a frame homomorphism.  

  If $\Frame$ restricts disclosure from $\lsrc$ to $\lobs$ to within
  $f$, then $\Frame'$ restricts disclosure from $h(\lsrc)$ to
  $h(\lobs)$ to within $g=h\circ f\circ h^{-1}$.
\end{theorem}
%
\begin{proof}
  We must show (1) that $g=h\circ f\circ h^{-1}$ is a blur function,
  and also (2) that the set $S$ of $h(\lsrc)$-runs compatible with any
  given $h(\lobs)$-run is $g$-blurred.

  \smallskip\noindent\textbf{1.}  The form of the definition
  guarantees the \emph{Inclusion} and \emph{Union} properties, so we
  only need to check \emph{Idempotence}, i.e.~$g\circ g=(h\circ f\circ
  h^{-1})\circ(h\circ f\circ h^{-1})=g$.  However, if $\bnd_1\in
  h^{-1}(h(\bnd_0))$, then $\bnd_0,\bnd_1$ are isomorphic.  Thus, by
  associativity:
%
  \begin{eqnarray*}
    g\circ g & = & (h\circ f\circ h^{-1})\circ (h\circ f\circ h^{-1})
    \\
    & = & h\circ f\circ f\circ h^{-1} \\ 
    & = & h\circ f\circ h^{-1} = g 
  \end{eqnarray*}
%
  since $f$ is idempotent.  
%

  \smallskip\noindent\textbf{2.}  Suppose $\bnd_{ho}$ is a
  $h(\lobs)$-run in $\Frame'$, and
  $\bnd_{hs}\in\cmpt{h(\lobs)}{h(\lsrc)}{\bnd_{ho}}$ is an
  $h(\lsrc)$-run.
%
  We must show that for any $\bnd_{hs}'\in g(\{\bnd_{hs}\})$,
  $\bnd_{hs}'\in\cmpt{h(\lobs)}{h(\lsrc)}{\bnd_{ho}}$ also.


  So let $\bndA_h\in\exec(\Frame')$ witness for
  $\bnd_{hs}\in\cmpt{h(\lobs)}{h(\lsrc)}{\bnd_{ho}}$.  By
  Def.~\ref{def:collapse}, Clause~\ref{cl:collapse:backward}, there is
  an $\bndA\in\exec(\Frame)$ such that $\bndA_h=h(\bndA)$.  By
  Lemma~\ref{lemma:frame:hom},
  $h({\restrict{\bndA}{\lobs}})={\bnd_{ho}}$ and
  $h({\restrict{\bndA}{\lsrc}})={\bnd_{hs}}$.

  The assumption on $\bnd_{hs}'$ says that $\bnd_{hs}'\in
  h(f(h^{-1}(\{\bnd_{hs}\})))$.  Using Lemma~\ref{lemma:frame:hom},
  $\bnd_{hs}'\in h(f({\restrict{\bndA}{\lsrc}}))$.  By
  Def.~\ref{def:collapse}, Clause~\ref{cl:collapse:forward} and
  Lemma~\ref{lemma:frame:hom}, there is a $\lsrc$-run $\bnd_s'\in
  f({\restrict{\bndA}{\lsrc}})$ such that $h(\bnd_s')=\bnd_{hs}'$.

  Since $\cmpt{\lobs}{\lsrc}{\restrict{\bndA}{\lobs}}$ is $f$-blurred,
  some $\bndA'$ witnesses for
  $\bnd_s'\in\cmpt{\lobs}{\lsrc}{\restrict{\bndA}{\lobs}}$.  Thus, by
  Lemma~\ref{lemma:frame:hom}, $h(\bndA')$ witnesses for
  $\bnd_{hs}'\in\cmpt{h(\lobs)}{h(\lsrc)}{\bnd_{ho}}$.  \myqed
%   
%   
%   
%   %
%     $$ \bnd_{hs}'\in h(f(h^{-1}(\{\bnd_{hs}\}))) \subseteq
%     h(f({\restrict{\bndA}{\lsrc}})), 
%     $$
%     and since $\bnd_{hs}'$ is an ${h(\lsrc)}$-run, there is
%     $\bndA_h'\in\exec(\Frame')$ such that
%     $\bnd_{hs}'=\restrict{\bndA_h'}{h(\lsrc)}$.  Using
%     Def.~\ref{def:collapse}, Clause~\ref{cl:collapse:backward} again,
%     there is a $\bndA'\in\exec(\Frame)$ such that $\bndA_h'=h(\bndA')$.
%     In particular, $\bnd_{hs}'=h(\restrict{\bndA'}{\lsrc})$.  Thus,
%     $\restrict{\bndA'}{\lsrc}\in f({\restrict{\bndA}{\lsrc}})$.  By
%     $\Frame$ restricts disclosure to within $f$,
%     $(\restrict{\bndA'}{\lsrc}) \in
%     \cmpt{\lobs}{\lsrc}{\restrict{\bndA}{\lobs}}$.
%   
%     Letting $\bndA''$ be a witness for this last compatibility, we have
%     $h(\bndA'')$ a witness for the desired
%     $\bnd_{hs}'\in\cmpt{h(\lobs)}{h(\lsrc)}{\bnd_{ho}}$, using
%     Def.~\ref{def:collapse}, Clause~\ref{cl:collapse:forward}.
%     \myqed
\end{proof}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "ccut"
%%% End: 


==> copyright_etc.tex <==
\thanks{\copyright\ 2014
  The MITRE Corporation.  All rights reserved.  Authors' email
  addresses:  \{guttman, prowe\}@mitre.org.  %Draft of \today.
}

\textsf{Approved for
  Public Release; Distribution Unlimited. \\
  Case Number 14-3139}

\paragraph{Notice.}  This technical data was produced for the US
Government under Contract No. W15P7T-13-C-A802, and is subject to the
Rights in Technical Data--Noncommercial Items clause at DFARS
252.227-7013 (Feb 2012).


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "ccut"
%%% End: 


==> hom.tex <==
\ifieee \subsection{Frame homomorphisms}\else\section{Frame homomorphisms}\fi
\label{sec:hom}

This appendix is included only for the convenience of the referees.
\ifblind\else See the technical report version on
\url{arxiv.org},~\cite{GuttmanRowe14:cut}.\fi 

Homomorphisms in general are structure-preserving maps, and frame
homomorphisms are maps that preserve both graph structure and also
executions.  Homomorphisms are useful for representing refinement
steps.  
%
\begin{definition}
  \label{def:hom}
  Suppose given frames
  $\Frame=(\Locations,\Channels,\mathcal{D},\pends,\ldots)$ and
  $\Frame'=(\Locations',\Channels',\mathcal{D}',\pends',\ldots)$.  Let
  $h=(h_{\Locations},h_{\Channels},h_{\mathcal{D}},h_{\runs})$, where
% 
  $$ h_L\colon\Locations\rightarrow\Locations', \quad
  h_C\colon\Channels\rightarrow\Channels', \quad
  h_D\colon\mathcal{D}\rightarrow\mathcal{D}',$$
%
  and $h_{\runs}\colon\ES(\Frame)\rightarrow\ES(\Frame')$.
%
  We apply $h$ to values using the relevant components, and lift $h$
  to sets, writing $h(C)$ for $\{h(c)\colon c\in
  C\}\subseteq\Channels'$, etc.
  \begin{enumerate}
    \item $h$ is a \emph{graph homomorphism}
    $h\colon\Frame\rightarrow\Frame'$ iff, for all $c\in\Channels$,
%
    $$h(\sender(c))=\sender(h(c))\ifieee$$\else\quad\mathrm\fi{and}
    \quad\ifieee$$\else\quad\fi h(\recipt(c))=\recipt(h(c)).$$
%   %
%       \begin{eqnarray*}
%         \entry(c)\in\pends(\ell)&\mathrm{implies} &
%         \entry(h(c))\in\pends(h(\ell)) \\
%         \exit(c)\in\pends(\ell)& \mathrm{implies} &
%         \exit(h(c))\in\pends(h(\ell)) .
%       \end{eqnarray*}
%
    \item A graph homomorphism $h$ is a \emph{frame homomorphism},
    written $h\colon\Frame\rightarrow\Frame'$, iff, for all
    $C\subseteq\Channels$ and $\bnd\in\lruns C(\Frame)$, 
    \begin{enumerate}
      \item $h(\bnd)\in\lruns {h(C)}(\Frame')$;\label{clause:hom:forward}
      \item for some $\preceq$-preserving
      $\phi\colon\events(\bnd)\rightarrow\events(h(\bnd))$, for all
      $e\in\events(\bnd)$,
%
      $$\chan(\phi(e))=h(\chan(e))\ifieee$$\else\quad\mathrm\fi{and}
      \quad\ifieee$$\else\quad\fi 
      \msg(\phi(e))=h(\msg(e));$$
      \item if $C_0\subseteq h^{-1}(C')\subseteq C$ and
      $h(C_0)\subseteq C'$, then \label{clause:hom:smooth}
%
      $$h(\restrict\bnd h^{-1}(C')) = \restrict{h(\bnd)}{C'}.
      \qquad\qquad\defsymbol$$ 
    \end{enumerate}
    %   
%   
%       \item Let $h\colon\Frame\rightarrow\Frame'$ be a graph
%       homomorphism, $C \subseteq\Channels$, $\bnd\in\lruns C(\Frame)$,
%       and $\bnd'\in\lruns{h(C)}(\Frame')$.  $\bnd'$ is an
%       $h,C$\emph{-image} of $\bnd$ iff for some $\preceq$-preserving map
%       $\phi\colon\events(\bnd)\rightarrow\events(\bnd')$, for all
%       $e\in\events(\bnd)$,
%   %
%       $$\chan(\phi(e))=h(\chan(e))\quad\mathrm{and} \quad
%       \msg(\phi(e))=h(\msg(e)).$$
%   %
%       $\hchan C(S)$ is the set of $h,C$-images of $\bnd\in
%       S\subseteq\lruns C(\Frame)$.  We write $\hchan C(*)$ for $\hchan
%       C(\lruns C(\Frame))$, and $h[*](*)$ for $\hchan{\Channels}(*)$.
%   %   
%   %
%       \item A graph homomorphism $h\colon\Frame\rightarrow\Frame'$ is a
%       \emph{frame homomorphism} iff for every $\bndA\in\exec(\Frame)$,
%       $\hchan{\Channels}(\{\bndA\})\not=\emptyset$.
%       \label{cl:hom:forward}  
%    \defend
  \end{enumerate}
%
\end{definition}
%
A homomorphism $h\colon\Frame\rightarrow\Frame'$ is \emph{onto} if the
functions $h_{\Locations},h_{\Channels},h_{\mathcal{D}},h_{\runs}$ are
surjective.  In this case, $\Frame$ exhibits finer structure than
$\Frame'$, which has ``forgotten'' structure from $\Frame$.  So
$\Frame$ is a kind of refinement of $\Frame'$.  When
$h\colon\Frame\rightarrow\Frame'$ is an \emph{embedding}, i.e.~its
functions are injective, there is more information and structure in
$\Frame'$.  Then we can consider $\Frame'$ to be a different kind of
refinement.
%
\begin{definition}
  Let $h\colon\Frame\rightarrow\Frame'$, and
  $C_1,C_2\subseteq\Channels$.  Then $h$ \emph{extends pre-images}
  from $C_1$ to $C_2$ iff, for all $\bnd_1\in\lruns{C_1}(\Frame)$ and
  $\bnd'\in\lruns{h(C_1)\cup h(C_2)}(\Frame')$, 
%   %
%     $$\bnd_1\in\lruns {C_1}(\Frame), \quad
%   %  \bnd_2'\in\lruns{h(C_2)}(\Frame'), \quad
%     \bnd'\in\lruns{(h(C_1)\cup h(C_2))}(\Frame'),$$
  if $\restrict{\bnd'}{h(C_1)}=h(\bnd_1)$,
      % $\bndA'$ witnesses for $\bnd'\in\cmpt{h(C)}{h(C')}{h(\bnd)}$,
  then there is a $\bnd\in\lruns{(C_1\cup C_2)}(\Frame)$ such that
  $\restrict\bnd{C_1}=\bnd_1$ and $h({\bnd})=\bnd'$.  \defend
%
\end{definition}
%
%
\begin{theorem}
  \label{thm:blur:hom} 
%
  Let $h\colon\Frame\rightarrow\Frame'$ and
  $\lsrc,\lobs\subseteq\Channels$; and assume
  \begin{enumerate}
    \item $h^{-1}(h(\lsrc))=\lsrc$ and $h^{-1}(h(\lobs))=\lobs$;
    \item $h$ is injective on $\lruns\lsrc$;
    \item $h$ extends pre-images from $\lsrc$ to $\lobs$.
  \end{enumerate}
%
  If $\Frame$ restricts disclosure from $\lsrc$ to $\lobs$ to within
  $f$, then $\Frame'$ restricts disclosure from $h(\lsrc)$ to
  $h(\lobs)$ to within the function $g$ such that:
%
  $$ g(S) = S\cup h(f(h^{-1}(S))).
  $$
%  
\end{theorem}
%
\begin{proof}  We must show that $g$ is a blur operator on
  $\lruns{h(\lsrc)}$, and then that the compatible sets are
  $g$-blurred.  

  \smallskip\noindent\textbf{1.}  The form of the definition
  guarantees the \emph{Inclusion} and \emph{Union} properties, so we
  only need to check \emph{Idempotence}.  Clearly, the union with $S$
  does not affect idempotence.  Thus, we want to show that $g\circ
  g=(h\circ f\circ h^{-1})\circ(h\circ f\circ h^{-1})=g$.  

  Since $h$ is injective on $\lruns\lsrc$, if $S\subseteq\lruns\lsrc$,
  then $h^{-1}(h(S))=S$.  Thus, by associativity and the idempotence
  of $f$:
%
  \begin{eqnarray*}
    g\circ g & = & (h\circ f\circ h^{-1})\circ (h\circ f\circ h^{-1})
    \\
    & = & h\circ f\circ f\circ h^{-1} \\ 
    & = & h\circ f\circ h^{-1} = g .
  \end{eqnarray*}
%

  \smallskip\noindent\textbf{2.}  Suppose that
  $\bnd_{hs}\in\cmpt{h(\lobs)}{h(\lsrc)}{\bnd_{ho}}$.  By the
  compatibility assumption, there is a $\bnd_h\in\lruns{(h(\lsrc)\cup
    h(\lobs))}$ such that $\restrict{\bnd_h}{h(\lsrc)}=\bnd_{hs}$ and
  $\restrict{\bnd_h}{h(\lobs)}=\bnd_{ho}$.

  Whenever $\bnd_{hs}'\in g(\{\bnd_{hs}\})$, we must show that
  $\bnd_{hs}'\in\cmpt{h(\lobs)}{h(\lsrc)}{\bnd_{ho}}$.  By the
  definition of $g$, either $\bnd_{hs}'\in \{\bnd_{hs}\}$ or else
  $\bnd_{hs}'\in h(f(h^{-1}(\{\bnd_{hs}\})))$.  In the first case, we
  are done.

  So assume the latter; thus, there exist $\bnd_s,\bnd_s'$ such that
  $h(\bnd_s)=\bnd_{hs}$, $h(\bnd_s')=\bnd_{hs}'$, and $\bnd_s'\in
  f(\{\bnd_s\})$.

  By the assumption that $h$ extends pre-images from $\lsrc$ to
  $\lobs$, there is a $\bnd\in\lruns{(\lsrc\cup\lobs)}(\Frame)$ such
  that $\restrict\bnd{\lsrc}=\bnd_s$ and $h({\bnd})=\bnd_h$.  Since
  $h^{-1}(h(\lobs))=\lobs$, Def.~\ref{def:hom},
  Clause~\ref{clause:hom:smooth} implies
  
%
  $$h(\restrict\bnd{\lobs})=\restrict{h(\bnd)}{h(\lobs)}= \bnd_{ho}.$$  
%
 
  Let $\bnd_o$ be $\restrict\bnd{\lobs}$.  Since $\bnd$ is a witness,
  $\bnd_s\in\cmpt{\lobs}{\lsrc}{\bnd_o}$.  By assumption, the
  compatible runs are $f$-blurred, so
  $\bnd_s'\in\cmpt{\lobs}{\lsrc}{\bnd_o}$.  Thus, there is a
  $\bnd'\in\lruns{(\lsrc\cup\lobs)}(\Frame)$ such that
  $\restrict{\bnd'}{\lsrc}=\bnd_s'$ and
  $\restrict{\bnd'}{\lobs}=\bnd_o$.  By Def.~\ref{def:hom},
  Clause~\ref{clause:hom:forward},
  $h(\bnd')\in\lruns{h(\lsrc\cup\lobs)}(\Frame')$.  Since
  $h^{-1}(h(\lsrc))=\lsrc$, by Clause~\ref{clause:hom:smooth},
%
  $$\restrict{h(\bnd')}{h(\lsrc)}=h(\restrict{\bnd'}\lsrc)=\bnd_{hs}'.$$
%
  Similarly, 
%
  $$ \restrict{h(\bnd')}{h(\lobs)} = h(\restrict{\bnd'}\lobs) =
  h(\bnd_o)= \bnd_{bo} . 
  $$
%
  So ${h(\bnd')}$ is a witness for
  $\bnd_{hs}'\in\cmpt{h(\lobs)}{h(\lsrc)}{\bnd_{ho}}$.  \myqed
%
\end{proof}


\iffalse paralipomena 


We would like to show that frame homomorphisms $h$ preserve some
security properties, but this is possible only if $h$ acts smoothly on
the channels involved, and on the blur operator that defines the
security properties.  
%
\begin{definition}
  Let $h$ be a frame homomorphism and $C,C'\subseteq\Channels$.
%
  \begin{enumerate}
    \item $C$ is \emph{stable under} $h$ iff $h^{-1}(h(C))=C$, and
    moreover, for all $\bnd\in\hchan C (*)$,
    $h(h^{-1}(\{\bnd\}))\subseteq \{\bnd\}$.
    \item $h$ \emph{extends pre-images} from $C$ to $C'$ iff, for all
    $\bnd_1,\bnd_2$,
    \begin{description}
      \item[if] $\bnd_1$ is an $h,C$-image, and $\bndA$ witnesses for
      $\bnd_2\in\cmpt{h(C)}{h(C')}{\bnd_1}$,
      \item[then] $\restrict\bndA{h(C)\cup h(C')}$ is an $h,{C\cup C'}$-image.
    \end{description}    
  \end{enumerate}  
\end{definition}
%
We now have our theorem giving a criterion for security preservation:
%
\begin{theorem}
  Let $h\colon\Frame\rightarrow\Frame'$ be a frame homomorphism; let
  $f$ on $\lruns \lsrc$ be stable under $h$; and let $h$ extend
  pre-images from $h(\lsrc)$ to $h(\lobs)$.

  If $\Frame$ restricts disclosure from $\lsrc$ to $\lobs$ to within
  $f$, then $\Frame'$ restricts disclosure from $h(\lsrc)$ to
  $h(\lobs)$ to within the function $g$ such that:
%
  $$ g(S) = S\cup h(f(h^{-1}(S))).
  $$
%  
\end{theorem}
%
\begin{proof}  We must show that $g$ is a blur operator on
  $\lruns{h(\lsrc)}$, and then that the compatible sets are
  $g$-blurred.  

  \smallskip\noindent\textbf{1.}

  \smallskip\noindent\textbf{2.}  Suppose that
  $\bnd_{hs}\in\cmpt{h(\lsrc)}{h(\lobs)}{\bnd_{ho}}$.  

  
\end{proof}


%  This is non-sensical with the current defn.  
%   \begin{lemma}\label{lemma:frame:hom}
%     If $\bnd\in\ES(\Frame)$ and $C\subseteq\Channels$, then
%     $h(\restrict{\bnd}C)=\{\restrict{\bnd'}{h(C)}\colon \bnd'\in
%     h(\bnd)\}$.
%   \end{lemma}
%


With our definitions, security properties are preserved under
collapse; i.e.~insecurity (information flow) is preserved under
refinement.
%
\begin{theorem}
  \label{thm:morphisms:preserve:blur}
  Let $h\colon\Frame\rightarrow\Frame'$ be a frame homomorphism.  

  If $\Frame$ restricts disclosure from $\lsrc$ to $\lobs$ to within
  $f$, then $\Frame'$ restricts disclosure from $h(\lsrc)$ to
  $h(\lobs)$ to within $g=h\circ f\circ h^{-1}$.
\end{theorem}
%
\begin{proof}
  We must show (1) that $g=h\circ f\circ h^{-1}$ is a blur function,
  and also (2) that the set $S$ of $h(\lsrc)$-runs compatible with any
  given $h(\lobs)$-run is $g$-blurred.

  \smallskip\noindent\textbf{1.}  The form of the definition
  guarantees the \emph{Inclusion} and \emph{Union} properties, so we
  only need to check \emph{Idempotence}, i.e.~$g\circ g=(h\circ f\circ
  h^{-1})\circ(h\circ f\circ h^{-1})=g$.  However, if $\bnd_1\in
  h^{-1}(h(\bnd_0))$, then $\bnd_0,\bnd_1$ are isomorphic.  Thus, by
  associativity:
%
  \begin{eqnarray*}
    g\circ g & = & (h\circ f\circ h^{-1})\circ (h\circ f\circ h^{-1})
    \\
    & = & h\circ f\circ f\circ h^{-1} \\ 
    & = & h\circ f\circ h^{-1} = g 
  \end{eqnarray*}
%
  since $f$ is idempotent.  
%

  \smallskip\noindent\textbf{2.}  Suppose $\bnd_{ho}$ is a
  $h(\lobs)$-run in $\Frame'$, and
  $\bnd_{hs}\in\cmpt{h(\lobs)}{h(\lsrc)}{\bnd_{ho}}$ is an
  $h(\lsrc)$-run.
%
  We must show that for any $\bnd_{hs}'\in g(\{\bnd_{hs}\})$,
  $\bnd_{hs}'\in\cmpt{h(\lobs)}{h(\lsrc)}{\bnd_{ho}}$ also.


  So let $\bndA_h\in\exec(\Frame')$ witness for
  $\bnd_{hs}\in\cmpt{h(\lobs)}{h(\lsrc)}{\bnd_{ho}}$.  By
  Def.~\ref{def:hom}, Clause~\ref{cl:hom:backward}, there is
  an $\bndA\in\exec(\Frame)$ such that $\bndA_h=h(\bndA)$.  By
  Lemma~\ref{lemma:frame:hom},
  $h({\restrict{\bndA}{\lobs}})={\bnd_{ho}}$ and
  $h({\restrict{\bndA}{\lsrc}})={\bnd_{hs}}$.

  The assumption on $\bnd_{hs}'$ says that $\bnd_{hs}'\in
  h(f(h^{-1}(\{\bnd_{hs}\})))$.  Using Lemma~\ref{lemma:frame:hom},
  $\bnd_{hs}'\in h(f({\restrict{\bndA}{\lsrc}}))$.  By
  Def.~\ref{def:hom}, Clause~\ref{cl:hom:forward} and
  Lemma~\ref{lemma:frame:hom}, there is a $\lsrc$-run $\bnd_s'\in
  f({\restrict{\bndA}{\lsrc}})$ such that $h(\bnd_s')=\bnd_{hs}'$.

  Since $\cmpt{\lobs}{\lsrc}{\restrict{\bndA}{\lobs}}$ is $f$-blurred,
  some $\bndA'$ witnesses for
  $\bnd_s'\in\cmpt{\lobs}{\lsrc}{\restrict{\bndA}{\lobs}}$.  Thus, by
  Lemma~\ref{lemma:frame:hom}, $h(\bndA')$ witnesses for
  $\bnd_{hs}'\in\cmpt{h(\lobs)}{h(\lsrc)}{\bnd_{ho}}$.  \myqed
%   
%   
%   
%   %
%     $$ \bnd_{hs}'\in h(f(h^{-1}(\{\bnd_{hs}\}))) \subseteq
%     h(f({\restrict{\bndA}{\lsrc}})), 
%     $$
%     and since $\bnd_{hs}'$ is an ${h(\lsrc)}$-run, there is
%     $\bndA_h'\in\exec(\Frame')$ such that
%     $\bnd_{hs}'=\restrict{\bndA_h'}{h(\lsrc)}$.  Using
%     Def.~\ref{def:hom}, Clause~\ref{cl:hom:backward} again,
%     there is a $\bndA'\in\exec(\Frame)$ such that $\bndA_h'=h(\bndA')$.
%     In particular, $\bnd_{hs}'=h(\restrict{\bndA'}{\lsrc})$.  Thus,
%     $\restrict{\bndA'}{\lsrc}\in f({\restrict{\bndA}{\lsrc}})$.  By
%     $\Frame$ restricts disclosure to within $f$,
%     $(\restrict{\bndA'}{\lsrc}) \in
%     \cmpt{\lobs}{\lsrc}{\restrict{\bndA}{\lobs}}$.
%   
%     Letting $\bndA''$ be a witness for this last compatibility, we have
%     $h(\bndA'')$ a witness for the desired
%     $\bnd_{hs}'\in\cmpt{h(\lobs)}{h(\lsrc)}{\bnd_{ho}}$, using
%     Def.~\ref{def:hom}, Clause~\ref{cl:hom:forward}.
%     \myqed
\end{proof}

\fi



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "ccut"
%%% End: 


==> refine.tex <==
\section{Security and Refinement}
\label{sec:refine} 

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "ccut"
%%% End: 


==> voting_eg.tex <==
\subsection{Two Applications}
\label{sec:cut:blur:applications}

Cor.~\ref{cor:compose} is an extremely useful compositional principle.
It implies, for instance in connection with Example~\ref{eg:cut:blur},
that non-exportable traffic in $n_1,n_2$ remains unobservable even as
we vary the top part of Fig.~\ref{fig:net:1}.
%
\begin{eg}
  \label{eg:compositional} 
  Regarding Fig.~\ref{fig:net:1} as the frame $\Frame_1$, let
  $\Frame_0$ be the part below $\{c_1,c_2\}$, and let
  $\lcut=\{c_1,c_2\}$.  Let $\Frame_2$ contain $\Frame_0,\lcut$ as
  shown, and have any graph structure above $\lcut$ such that $\lcut$
  remains a cut between the new structure and $\Frame_0$.  Let the new
  locations have any transition systems such that the local runs
  agree, i.e.~$\lruns\lcut(\Frame_2)=\lruns\lcut(\Frame_1)$.
%
  Then by Cor.~\ref{cor:compose}, external observations of
  $\chans(\{n_1,n_2\})$ are guaranteed to blur out non-exportable
  events.  \defend
\end{eg}
%
It is appealing that our security goal is independent of changes in
the structure of the internet that we do not control.  A similar
property holds for the integrity goal of Example~\ref{eg:cut:blur} as
we alter the internal network.  The converse questions---preserving
the confidentiality property as the internal network changes, and the
integrity property as the internet changes---appear to require a
different theorem.  Thm.~\ref{thm:blur:hom} in Appendix~\ref{sec:hom}
is intended to handle these questions.

\begin{eg}
  \label{eg:voting:compositional}
%
  Consider a frame representing a precinct, of the form shown in
  Fig.~\ref{fig:precinct}.  
%
  \begin{figure}
    \centering
    place figure here.  
    \caption{A single precinct}
    \label{fig:precinct}
  \end{figure}
%
\end{eg}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "ccut"
%%% End:

